Discovering Gender Differences in Facial Emotion Recognition via Implicit Behavioral Cues

We examine the utility of implicit behavioral cues in the form of EEG brain signals and eye movements for gender recognition (GR) and emotion recognition (ER). Specifically, the examined cues are acquired via low-cost, off-the-shelf sensors. We asked 28 viewers (14 female) to recognize emotions from unoccluded (no mask) as well as partially occluded (eye and mouth masked) emotive faces. Obtained experimental results reveal that (a) reliable GR and ER is achievable with EEG and eye features, (b) differential cognitive processing especially for negative emotions is observed for males and females and (c) some of these cognitive differences manifest under partial face occlusion, as typified by the eye and mouth mask conditions.

==> GRnVR.tex <==
We examined EEG responses and gaze features (also their fusion) corresponding to HI morphs with no mask and masked conditions for emotion(valence) and gender recognition(both emotion wise and across emotions). We have used the ten features--saccade orientation, histogram of saccade slope, histogram of saccade length,histogram of saccade velocity, histogram of fixation duration, fixation histogram, top-ten salient coordinates, saliency histogram and saliency map to form feature vector of 825 length as explained in \cite{Tavakoli15} from the fixations and saccades of eye tracking data.The data is subjected to PCA to retain 90\% variance. Classifiers used include Naive Bayes(NB), Linear Discriminant Analysis(LDA) and Support Vector Machines with RBF(RSVM) and linear kernels(LSVM). We have opted for area under ROC curve(AUC) metric to evaluate the classifiers, since it is robust to class imbalance that might occur in case of valence recognition. Only the best among the classification results are presented and the corresponding classifier is mentioned.

\subsubsection{Valence Recognition}
ER(valence) has been carried out as classification of positive emotions(happy and surprise) and negative emotions(anger, disgust, fear and sad). It is implicit that the classification is unbalanced and thus our choice of AUC as metric is appropriate. A 5 repetitions of 10 fold cross validation has been used for classification after PCA to retain 90\% variance in the data. The classifiers employed are NB, LDA, RSVM and LSVM.

Figure-\ref{Fix_dur_dist} presents ER results for males and females for various morphs. Among all the modalities, the best performance(females-0.63 and males-0.64 with LDA) is achieved with eye tracking data for no mask condition, which is better than the performance(accuracy-50.7\%) achieved by \cite{Tavakoli15}. Though a close to chance performance is achieved using with EEG responses(AUC--0.54), it is apparent since previous works\cite{abadi2015decaf,Muhl14} reported a 60\% valence recognition using lab-grade sensors. The ER for masked stimuli is observed to be at chance level using EEG or eye tracking data but the fusion methods have achieved above chance results. It can observed that the performance for females is better than males for no mask and lower half masked morphs (strongly observable for early fusion). For upper half masked stimuli, though the difference between females and males is negligible, the early fusion results show that males are better at ER when lower part is visible, this can be justified from \cite{wells2016identification} that males attend more to mouth than females.


\subsubsection{Gender Recognition}
\input{gender_table_comp}

\begin{figure*}
\includegraphics[width=0.245\textwidth]{SVM_win_gender_recogn_HIcor_AUCnew1}
\includegraphics[width=0.245\textwidth]{win_GR_eyemaksed}
\includegraphics[width=0.245\textwidth]{win_GR_mouthmaksed} \hspace{0.1cm}
\includegraphics[width=0.24\textwidth]{spatio_comp_lab} \vspace{-.1cm}
\centerline{(a)\hspace{0.23\linewidth}(b)\hspace{0.23\linewidth}(c)\hspace{0.23\linewidth}(d)}
\caption{(a--c): Temporal variance in GR performance for the \textit{no mask}, \textit{eye mask} and \textit{mouth mask} conditions. (d) Top three electrodes showing best GR performance for the three conditions.}
\label{winGRnVR}
\end{figure*}

Prior works have attempted GR using EEG responses for no mask faces and achieved 97.1\% accuracy using lab-grades sensors. We have achieved 0.71 AUC for no mask morphs using the low cost Emotiv device with low SNR(classifier mentioned in the table). It can be observed from table-\ref{GenResults} that the GR performance on par with no mask morphs can be achieved for masked morphs. While our attempt to perform GR with Eye tracking data gave chance level performance, the Late fusion of decisions still out performed than Early fusion. 5 repetitions of 10 fold cross validation with was used to classify the data after it has been subjected to dimensionality reduction.

Emotion wise GR using different modalities have been presented in table-\ref{GenResults} and it can observed that the GR using EEG responses out preform the other modalities. The highest GR is attained for anger and least for fear. This trend is consistent for masked morphs also. While Anger being most discriminative emotion between males and females, a significant performance drop can be noticed when upper half masked stimuli are presented over lower masked morphs. This is expected based on previous findings\cite{schurgin}. Fear is observed to perform better at discriminating genders with upper half masked morphs than lower half visible are presented. \textit{Schurgin et al} also observed that the recognition of happy was best for upper masked morphs, this is supported by a strong difference between GR using upper masked morphs and lower masked morphs by Early fusion and no significant differences were observed in GR for sad with either of the masks being used.

Figure-\ref{winGRnVR} shows GR results from dividing the post stimuli epochs into 4 windows of uniform duration. No significant emotion differences in GR are observed for no mask scenario. The performance for masked scenario is less than that of no masked counterpart for most emotions(as in the case of the non-window approach in table-\ref{GenResults}). In addition, anger remains best discriminative emotion during the temporal analysis (AUC--0.78). While surprise performs better for upper than lower half masked morphs, we can notice that the RR for surprise is higher for upper masked than lower masked morphs.

A spatial analysis for GR has been performed to identify the important(top-3 and bottom-3) electrode locations out of the 14 available ones. We have used the RSVM with same cross validation settings as described in the previous analysis to rank the electrodes for all three kinds of morphs for epochs corresponding to 1s post stimuli presentation.

We observe from figure-\ref{winGRnVR}, that GR for masked morphs is better than no mask morphs in contrast, the performance of least performing electrodes has deteriorated for masked condition. The best performing electrode locations for no mask morphs are F8(0.55),T7 and AF4 while the least performing are F3,O2 and AF3(0.23). The best performing electrode locations for upper half mask morphs are O2(0.87),P7 and FC6 while the least performing are O1,FC5 and F7(0.03). The best performing electrode locations for lower half mask morphs are F3(0.89),P7 and O1 while the least performing are AF4,O2,FC5(0.06).

From above results, it can be inferred that the best performing electrodes for no mask and upper half masked stimuli correspond to right hemisphere of brain and least performing electrodes to left hemisphere of the brain. The scenario is opposite for lower half masked stimuli. This is just a pattern we have observed and we have not encountered any literature that supports this statement.


